Camera Control for Text-to-Image Generation via Learning Viewpoint Tokens

Current text-to-image models struggle to provide precise camera control using natural language alone. In this work, we present a framework for precise camera control with global scene understanding in text-to-image generation by learning parametric camera tokens. We fine-tune image generation models for viewpoint-conditioned text-to-image generation on a curated dataset that combines 3D-rendered images for geometric supervision and photorealistic augmentations for appearance and background diversity. Qualitative and quantitative experiments demonstrate that our method achieves state-of-the-art accuracy while preserving image quality and prompt fidelity. Unlike prior methods that overfit to object-specific appearance correlations, our viewpoint tokens learn factorized geometric representations that transfer to unseen object categories. Our work shows that text-vision latent spaces can be endowed with explicit 3D camera structure, offering a pathway toward geometrically-aware prompts for text-to-image generation. Project page: https://randdl.github.io/viewtoken_control/

==> output/multi_pitch_yaw/pitch_yaw_table.tex <==
\begin{table}[h]
\centering
\caption{Pitch and yaw variation results. Main 3×3 grid shows radius=4.5, extra row and column show radius=6.0.}
\label{tab:pitch_yaw}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{c|ccc|c}
\hline
Pitch $\backslash$ Yaw & -10° & 0° & 10° & 0° (r=6) \\
\hline
-10° &
\includegraphics[width=0.18\textwidth]{qualitative_results/multi_pitch_yaw/az+055.00_el+15.00_r+4.50_p-10.00_y-10.00.jpg} &
\includegraphics[width=0.18\textwidth]{qualitative_results/multi_pitch_yaw/az+055.00_el+15.00_r+4.50_p-10.00_y+00.00.jpg} &
\includegraphics[width=0.18\textwidth]{qualitative_results/multi_pitch_yaw/az+055.00_el+15.00_r+4.50_p-10.00_y+10.00.jpg} &
\includegraphics[width=0.18\textwidth]{qualitative_results/multi_pitch_yaw_radius_6/az+055.00_el+15.00_r+6.00_p-10.00_y+00.00.jpg} \\
\hline
0° &
\includegraphics[width=0.18\textwidth]{qualitative_results/multi_pitch_yaw/az+055.00_el+15.00_r+4.50_p+00.00_y-10.00.jpg} &
\includegraphics[width=0.18\textwidth]{qualitative_results/multi_pitch_yaw/az+055.00_el+15.00_r+4.50_p+00.00_y+00.00.jpg} &
\includegraphics[width=0.18\textwidth]{qualitative_results/multi_pitch_yaw/az+055.00_el+15.00_r+4.50_p+00.00_y+10.00.jpg} &
\includegraphics[width=0.18\textwidth]{qualitative_results/multi_pitch_yaw_radius_6/az+055.00_el+15.00_r+6.00_p+00.00_y+00.00.jpg} \\
\hline
10° &
\includegraphics[width=0.18\textwidth]{qualitative_results/multi_pitch_yaw/az+055.00_el+15.00_r+4.50_p+10.00_y-10.00.jpg} &
\includegraphics[width=0.18\textwidth]{qualitative_results/multi_pitch_yaw/az+055.00_el+15.00_r+4.50_p+10.00_y+00.00.jpg} &
\includegraphics[width=0.18\textwidth]{qualitative_results/multi_pitch_yaw/az+055.00_el+15.00_r+4.50_p+10.00_y+10.00.jpg} &
\includegraphics[width=0.18\textwidth]{qualitative_results/multi_pitch_yaw_radius_6/az+055.00_el+15.00_r+6.00_p+10.00_y+00.00.jpg} \\
\hline
0° (r=6) &
\includegraphics[width=0.18\textwidth]{qualitative_results/multi_pitch_yaw_radius_6/az+055.00_el+15.00_r+6.00_p+00.00_y-10.00.jpg} &
\includegraphics[width=0.18\textwidth]{qualitative_results/multi_pitch_yaw_radius_6/az+055.00_el+15.00_r+6.00_p+00.00_y+00.00.jpg} &
\includegraphics[width=0.18\textwidth]{qualitative_results/multi_pitch_yaw_radius_6/az+055.00_el+15.00_r+6.00_p+00.00_y+10.00.jpg} &
 \\
\hline
\end{tabular}
}
\end{table}


==> qualitative_results/multi_pitch_yaw/pitch_yaw_table.tex <==
\begin{table}[h]
\centering
\caption{Pitch and yaw variation results. Main 3×3 grid shows radius=4.5, extra row and column show radius=6.0.}
\label{tab:pitch_yaw}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{c|ccc|c}
\hline
Pitch $\backslash$ Yaw & -10° & 0° & 10° & 0° (r=6) \\
\hline
-10° &
\includegraphics[width=0.18\textwidth]{qualitative_results/multi_pitch_yaw/az+055.00_el+15.00_r+4.50_p-10.00_y-10.00.jpg} &
\includegraphics[width=0.18\textwidth]{qualitative_results/multi_pitch_yaw/az+055.00_el+15.00_r+4.50_p-10.00_y+00.00.jpg} &
\includegraphics[width=0.18\textwidth]{qualitative_results/multi_pitch_yaw/az+055.00_el+15.00_r+4.50_p-10.00_y+10.00.jpg} &
\includegraphics[width=0.18\textwidth]{qualitative_results/multi_pitch_yaw_radius_6/az+055.00_el+15.00_r+6.00_p-10.00_y+00.00.jpg} \\
\hline
0° &
\includegraphics[width=0.18\textwidth]{qualitative_results/multi_pitch_yaw/az+055.00_el+15.00_r+4.50_p+00.00_y-10.00.jpg} &
\includegraphics[width=0.18\textwidth]{qualitative_results/multi_pitch_yaw/az+055.00_el+15.00_r+4.50_p+00.00_y+00.00.jpg} &
\includegraphics[width=0.18\textwidth]{qualitative_results/multi_pitch_yaw/az+055.00_el+15.00_r+4.50_p+00.00_y+10.00.jpg} &
\includegraphics[width=0.18\textwidth]{qualitative_results/multi_pitch_yaw_radius_6/az+055.00_el+15.00_r+6.00_p+00.00_y+00.00.jpg} \\
\hline
10° &
\includegraphics[width=0.18\textwidth]{qualitative_results/multi_pitch_yaw/az+055.00_el+15.00_r+4.50_p+10.00_y-10.00.jpg} &
\includegraphics[width=0.18\textwidth]{qualitative_results/multi_pitch_yaw/az+055.00_el+15.00_r+4.50_p+10.00_y+00.00.jpg} &
\includegraphics[width=0.18\textwidth]{qualitative_results/multi_pitch_yaw/az+055.00_el+15.00_r+4.50_p+10.00_y+10.00.jpg} &
\includegraphics[width=0.18\textwidth]{qualitative_results/multi_pitch_yaw_radius_6/az+055.00_el+15.00_r+6.00_p+10.00_y+00.00.jpg} \\
\hline
0° (r=6) &
\includegraphics[width=0.18\textwidth]{qualitative_results/multi_pitch_yaw_radius_6/az+055.00_el+15.00_r+6.00_p+00.00_y-10.00.jpg} &
\includegraphics[width=0.18\textwidth]{qualitative_results/multi_pitch_yaw_radius_6/az+055.00_el+15.00_r+6.00_p+00.00_y+00.00.jpg} &
\includegraphics[width=0.18\textwidth]{qualitative_results/multi_pitch_yaw_radius_6/az+055.00_el+15.00_r+6.00_p+00.00_y+10.00.jpg} &
 \\
\hline
\end{tabular}
}
\end{table}

